Multivariate Power Series in Maple

We present MultivariatePowerSeries, a Maple library introduced in Maple 2021, providing a variety of methods to study formal multivariate power series and univariate polynomials over such series. This library offers a simple and easy-to-use user interface. Its implementation relies on lazy evaluation techniques and takes advantage of Maple's features for object-oriented programming. The exposed methods include Weierstrass Preparation Theorem and factorization via Hensel's lemma. The computational performance is demonstrated by means of an experimental comparison with software counterparts.

==> acknowledgements.tex <==
%% Acknowledgements
\subsection*{Acknowledgements}



==> benchmarks.tex <==
\section{Experimentation}


==> powerseries_object.tex <==
% Implementing Power Series Arithmetic
\section{Implementing Power Series Arithmetic}
To achieve a lazy and high-performance implementation of multivariate power series, we develop a variety of facilities and methods. In this section, we start with a deeper look into the {\PSO} local members, introduce an efficient way to track the parents' objects utilized in the power series arithmetic, and describe I/O methods and other operators.
%%

%%
The first local member in Listing \ref{lst:PSO} is a mutable array of computed homogeneous parts ({\tt hpoly}). The size of array is increased when we need a homogeneous part of a degree larger than {\tt deg}. The value of {\tt deg} equals {\tt upperbound(hpoly)}, unless the difference between a requested homogeneous part and {\tt deg} is non-negligible. In this case, we reallocate {\tt hpoly} once and call the generator ({\tt gen}) to fill the array successively for the sake of efficiency.
%%

%%
The arithmetic generators are highly dependent on generators of inputs. For example, addition (or subtraction) of $f, g \in \KXN$ in Equation \ref{eq:pso-add} is actually the addition (or subtraction) of $f, g$ generators. So, we always need to keep a track of parents' objects. An optimized way to do is storing pointers of those input objects as {\tt ancestors} and utilize them when needed. 
%%

%%
As mentioned in the previous chapter, {\PSO} provides an advanced display style to represent a power series object. The analytical expression member of an object, {\tt algexpr}, stores the convergent if exists, and we mainly use it as a helper in methods {\tt Display} and {\tt ModulePrint}. We also create a new type for {\PSO} display style named {\tt PSDS\_TYPE} to control the maximum number of terms and precision which will be shown. 
%%

%%
There are three methods to create a power series object: {\tt PowerSeries}, {\tt GeometricSeries}, and {\tt SumOfAllMonomials}. {\tt PowerSeries} creates a new object from a polynomial, algebraic expression, or procedure. The other two methods create multivariate geometric series and sum of all monomials respectively. We also implement {\tt ModuleDeconstruct} to automatize the deconstruction. 
%%

%% 
The method {\tt Add} is a {\it n-ary} operator, and creates a generator for a sequence of {\PSO}, polynomials, and algebraic expressions with coefficients. The method {\tt Subtract} and {\tt Negate} compute the subtract of two objects and negate one. The method {\tt Multiply} is also a {\it n-ary} operator. The {\tt Divide} compute exact quotient of two objects. The listing \ref{lst:div} shows the implementation of this method in {\PSO}. Note {\tt AUTO\_EXPAND} is a local macro in {\MPS} and performs expansion efficiently supporting algebraic inputs. We also implement {\tt Inverse} and {\tt Exponentiate}. 
% The listing \ref{lst:mul} shows a high-level view of this method. Note our first try was with taking advantage of {\tt Iterators} but we got slow down due to intensively usage of {\tt expand} and {\tt Algebraic:-Expand} {\Maple} commands.
%% 
%%
\begin{lstlisting}[language = Maple, caption = {The division method in {\PSO}}, label={lst:div}]
export Divide ::static := proc(a, b, $)
	if HomogeneousPart(b,0) = 0 then 
		error "invalid input: not invertible"; 
	end if;
	local dummy;
	local hpoly := Array(0..0, [AUTO_EXPAND(dummy, 
				normal(HomogeneousPart(a,0)/
				HomogeneousPart(b,0)))]);
	return Object(PowerSeriesObject, hpoly, 0, div_gen, 
					["A" = a, "B" = b], # ancestors
					a:-algexpr/b:-algexpr); # algexp
end proc;
\end{lstlisting}
%%
%%
\begin{lstlisting}[language = Maple, caption = {The division generator in {\PSO}}, label={lst:divgen}]
local div_gen ::static := proc(a, d::nonnegint, $)
	local i, dummy;	
	local s := HomogeneousPart(a:-ancestors:-A, d);
	s -= add(AUTO_EXPAND(dummy, 
				HomogeneousPart(a:-ancestors:-B, i) *
				HomogeneousPart(a, d-i), i = 1..d);
	return AUTO_EXPAND(dummy, normal(s/
				 a:-ancestors:-B:-hpoly[0]));
end proc;
\end{lstlisting}

==> upops_object.tex <==
% Implementing UPoPS Arithmetic
\section{Implementing UPoPS Arithmetic}
We went through the implementation details of {\PSO} in the previous chapter. In this chapter, we study an important application of formal power series which is defined as univariate polynomials with multivariate power series coefficients and denoted as UPoPS. 
%%

%%
The {\UPoPSO} is a simple dense univariate polynomial which is developed as an {\tt Array} of {\PSO}s. The basic arithmetic algorithms, e.g. add, subtract, negate, and multiply, is naively achievable from {\PSO}. This implementation is lazy, as every basic arithmetic is automatically lazy through using {\PSO} routines. 
%%

%%
For example, the addition of two UPoPS objects $f = \sum_{i = 0}^{k} a_i Y^i$ and $g = \sum_{i=0}^{k} b_i Y^i$ in $\KXN[Y]$ is the summation $(a_i + b_i)Y^i$ for all $ 0 \leq i \leq k$ where $a_i, b_i$ are two {\PSO} objects. The same for other basic arithmetic, their implementation is inherited naively from the coefficient ring. 
%%

%%
However, there are important operations on UPoPS which are not straightforwardly achievable from power series arithmetic. In the following we explain lazy implementation of Weierstrass Preparation, Taylor Shift, and Factorization via Hensel's lemma in {\UPoPSO}. 
%%
\subsection*{Weierstrass Preparation}
Assume $f, p, \alpha \in \KXN[Y]$ where $f = \sum_{i = 0}^{d + m} a_i Y^i$, $p = Y^d + \sum_{i=0}^{d-1} b_i Y^i$, and $\alpha = \sum_{i=0}^{m} c_i Y^i$. We have $f = p \alpha$ from an extension of Theorem \ref{thm:WPT} over $\KXN[Y]$. From the proof, $f, p, \alpha$ must imply the following system of equations: 
%%

%%
\begin{equation}
\label{eq:WPT}
1: \begin{cases} \begin{array}{lcl} 
	{\color{persianblue} a_0} & = & \  {\color{persianred} b_0} { c_0} \\
	{\color{persianblue} a_1} & = & \ b_0 c_1 + {\color{persianred}  b_1} { c_0} \\
	    & \vdots &  \\
	{\color{persianblue} a_{d-1}} & = & \ b_0 c_{d-1} + b_1 c_{d-2} + \cdots + b_{d-2} c_1 + {\color{persianred} b_{d-1}} { c_0} 
	\end{array} \end{cases} 
\end{equation}
\begin{equation*}
2: \begin{cases} \begin{array}{lcl} 
	{\color{persianblue}  a_d} & = & \ b_0 c_d + b_1 c_{d-1} + \cdots + b_{d-1} c_1 + {\color{persianred} c_0} \ \ \ \ \  \\ 
	    & \vdots &  \\
	{\color{persianblue} a_{d+m-1}} & = & b_{d-1} c_{m} + {\color{persianred} c_{m-1}} \\
	{\color{persianblue} a_{d+m}}  & = & {\color{persianred} c_m} 
\end{array} \end{cases}
\end{equation*}
%%

%%
To solve these equations modulo successive powers of $\M$, the maximal ideal of $\KXN$, we will iteratively compute new homogenous parts of each power series $\{b_0, \ldots, b_{d-1}\}$ by Equations \ref{eq:WPT} (Part 1) and $\{c_0, \ldots, c_m\}$ by  Equations \ref{eq:WPT} (Part 2).
%%

%%
Consider that $b_0, \ldots, b_{d-1}, c_0, \ldots, c_{m}$ are known modulo $\M^r$ and $a_0, \ldots, a_{d-1}$ are known modulo $\M^{r+1}$. From the first equation in part $1$, homogeneous part $b_0$ modulo $\M^{r+1}$ can be computed. Then, the $a_1 - b_0 c_1$ becomes known modulo $\M^{r+1}$ as $\HomoPart{b_0, 0} = 0$ by definition, and $b_1$ can be solved in the equation $a_1 - b_0 c_1 = b_1 c_0$. We compute all $b_{2}, \ldots, b_{d-1}$ modulo $\M^{r+1}$ with the same argument.
%%

%%
After determining $b_0, \ldots, b_{d-1}$ modulo $\M^{r+1}$, we now can compute $c_m, c_{m-1}\ldots, c_0$ modulo $\M^{r+1}$ with a rearrangement of the equations (Part $2$) iteratively from bottom to up. As yet, we have seen how the coefficients of $p, \alpha$ will be updated by determining the homogeneous parts of successive degrees. Therefore, a lazy implementation of WPT requires a generator to update all coefficients simultaneously. Algorithm \ref{alg:WPupdate} shows our design of the generator that covers both phases.
%%
\begin{algorithm}[H]
	\caption{
		\small \textbf{WeierstrassUpdate}$(p, \alpha, F, r)$\newline
		Given $p = Y^d + \sum_{i=0}^{d-1} b_i Y^{i}$, $\alpha = \sum_{i=0}^{m} c_i Y^i$, and $\F = \{ F_i \vert F_i = a_i - \sum_{j=0}^{i-1} b_{j} c_{i-j}, i = \{0, \ldots, d-1 \}$ are all known modulo $M^{r}$, returns $b_0, \ldots, b_{d-1}, c_0, \ldots, c_m$ modulo $M^{r+1}$.} \label{alg:WPupdate}
	\begin{algorithmic}[1]
		\Statex {$\verb|#|$ denoted {\tt hpart} as {\tt HomogeneousPart}}
		\Statex {$\verb|#|$ update $b_0, ..., b_{d-1}$ modulo $M^{r+1}$} 
		\For{$i$ \textbf{from} $0$ \textbf{to} $d-1$}
		\State $s := \text{\tt add}(\text{\tt seq}( {\tt hpart}(b_i, r-k) * {\tt hpart}(c_{_0}, k), \ k =  1 \ .. \ r-1 ))$;
		\State ${\tt hpart}(b_i, r) := ({\tt hpart}(F_i, r) - s)/{\tt hpart}(c_0, 0)$;
		\EndFor
		\Statex {$\verb|#|$ ensure $c_0, ..., c_{m}$ are updated modulo $M^{r+1}$} 
		\For{$i$ \textbf{from} $0$ \textbf{to} $m$}
		\State ${\tt hpart}(c_i, r)$; 
		\EndFor	
	\end{algorithmic}
\end{algorithm}
%%
However, the question we have not explained yet is the way we initialize $p, \alpha$ before calling the generator. 
The main degree of $p$ will be simply determined through finding the first unit power series among $a_0, \ldots, a_{d+m}$. If $d = 0$, then $p = 1$ and $\alpha = f$, otherwise, $m = \deg(f) - d$, and we initialize $b_i$ with $\HomoPart{a_i, 0}$ for $ 0 \leq i \leq d-1$. Then, {\PSO} $c_m, \ldots, c_0$ can be created with basic power series arithmetic and equations in part $2$. 
%%

%%
In order to update the coefficients of $p$, we frequently need to compute the $a_i - \sum_{j=0}^{i-1} b_{j} c_{i-j}$ for every $0 \leq i \leq d-1$ as it explained before. To optimize this effort and reduce the creation time to once, we create these helper {\PSO} objects in advanced as the set $\F = \{ F_i \vert F_i = a_i - \sum_{j=0}^{i-1} b_{j} c_{i-j}, i = 0, \ldots, d-1 \}$ and passed them as ancestors of $b_0, \ldots, b_{d-1}$. (see Algorithm \ref{alg:WPupdate})
%%
%%
\subsection*{Taylor Shift}
The Taylor Shift operation takes a UPoPS object $f \in \KXN[Y]$ and does shifting $Y \rightarrow Y + c$, e.i. $f(Y+c)$, for some $c \in \K$. In our implementation, $c$ can be a {\tt numeric} or {\tt algebraic} types with the purpose of using efficiently in the factorization via Hensel's Lemma. However, this is basically well-defined for any element of the ring $\KXN$.
%%

%%
Assume $f = \sum_{i=0}^{k} a_i Y^i$ a multivariate power series in $\KXN[Y]$ and $c \in \K$. As the {\PSO} objects $a_0, \ldots, a_k$ are lazy power series, we want to make $f(Y+c)$ lazy. It means that we need to create a generator for the return power series. Let $\T = (t_{i,j})$ be the lower triangular matrix of the coefficients of $Y^j$ in the binomial expansion $(Y+c)^i$, for $0 \leq i \leq k$, and $0 \leq j \leq i$. Let $\{ b_0, \ldots, b_{k} \}$ be the list of coefficients of $f(Y+c)$ in {\KXN}. Then, it will be easy to prove that for every $0 \leq i \leq k$,  $b_i$ is the inner product of the $i$-th sub-diagonal of $\T$ with the lower $k+1-i$ elements of $\{ a_0, \ldots, a_k \}$.
%%

%%
After creating a lower triangular matrix $(k+1) \times (k+1)$ of $(Y+c)^i$ coefficients, for every $0 \leq i \leq k$. We can construct generators for $b_0, \ldots, b_k$ with taking advantage of $n$-ary addition algorithm in {\PSO}. Therefore, $f(Y+c) = \sum_{i=0}^{k} b_i Y^i$ will truly be a lazy UPoPS object in $\KXN[Y]$. 
%%
\subsection*{Factorization via Hensel's Lemma}
We have seen the Hensel's lemma for factorizing univariate polynomials over power series. Assume a UPoPS object $f \in \KXN[Y]$ and $r \in \N$. Here, we introduce a lazy algorithm based on the proof of Theorem \ref{thm:HF}, which can be found in \cite{CASC20}. This algorithm provides mechanism with making use of Taylor Shift and Weierstrass preparation algorithms to factor $f$ recursively (obtaining one factor at a time) into $f_1, \ldots, f_r$.
%%

%% 
Algorithm \ref{alg:fact} shows this procedure which begins by factorizing $f_{X \rightarrow 0} = f(0, \ldots, 0, Y)$ in $\K[Y]$. Note we call $f_{X \rightarrow 0}$ as {\tt EvaluateAtOrigin} method in our package. We also factor $f_{X \rightarrow 0}$ with taking advantage of fast routines in {\tt SolveTools} package in {\Maple} that let us to make a high-performance support for algebraic roots as well. Notice that the algorithm is lazy as it basically utilizes lazy UPoPS arithmetic. It also provides the concurrency opportunity with {\it pipelining} of Taylor shift and Weierstrass preparation calls in the for-loop. 
%%

%%
Assume $c_1^{k_1} \cdots c_r^{k_r}$ be the unique factorization of $f_{X \rightarrow 0}$ in $\K[Y]$. For simplicity of presentation, let us assume that $c_1, \ldots, c_r$ are linear factors over $\K$. To describe one step of the recursion in Algorithm \ref{alg:fact}, assume $f^{*}$ be the current polynomial to factorize. For a root $c_i$ of $f_{X \rightarrow 0}^{*}$, we perform a Taylor shift to obtain $g = f^{*}(Y + c_i)$. Then, we apply Weierstrass preparation to obtain $p, \alpha$ where $p$ is monic of degree $k_i$. Again, with using Taylor Shift, we reverse $p$ to obtain $f_i = p(Y - c_i)$, a factor of $f$, and $f^{*} = \alpha(Y - c_i)$, for the next iteration. 
%%
\begin{algorithm}[H]
	\caption{
		\small \textbf{HenselFactorize}$(f)$\newline
		Given $f = \sum_{i=0}^{k} a_i Y^{i} \in \KXN[Y]$, returns the list of factors $\{ f_1, \ldots, f_r \}$ satisfying the theorem (Factorization via Hensel's Lemma).} \label{alg:fact}
	\begin{algorithmic}[1]
		\State $f^{*} := f$; 
		\State $c_1, \ldots, c_r := \text{\tt Roots}(\bar{f}, Y)$;
		\For{$i$ \textbf{from} $1$ \textbf{to} $r$}
			\State $g := \text{\tt TaylorShift}(f^*, c_i)$;
			\State $p, \alpha := \text {\tt WeierstrassPreparation}(g)$;
			\State $f_i := \text{\tt TaylorShift}(p, -c_i)$;
			\State $f^* := \text{\tt TaylorShift}(\alpha, -c_i)$;
		\EndFor
		\State \Return $\{ f_1, \ldots, f_r \}$;
	\end{algorithmic}
\end{algorithm}
%\section{{\MPS} Package}
%
